Enhancing End-to-End Autonomous Driving with Latent World Model

In autonomous driving, end-to-end planners directly utilize raw sensor data, enabling them to extract richer scene features and reduce information loss compared to traditional planners. This raises a crucial research question: how can we develop better scene feature representations to fully leverage sensor data in end-to-end driving? Self-supervised learning methods show great success in learning rich feature representations in NLP and computer vision. Inspired by this, we propose a novel self-supervised learning approach using the LAtent World model (LAW) for end-to-end driving. LAW predicts future scene features based on current features and ego trajectories. This self-supervised task can be seamlessly integrated into perception-free and perception-based frameworks, improving scene feature learning and optimizing trajectory prediction. LAW achieves state-of-the-art performance across multiple benchmarks, including real-world open-loop benchmark nuScenes, NAVSIM, and simulator-based closed-loop benchmark CARLA. The code is released at https://github.com/BraveGroup/LAW.

==> tables/abl_carla.tex <==
\begin{wraptable}{r}{0.53\textwidth} 
\centering
\caption{\textbf{Ablation study on latent prediction on Town05 Long benchmark.}}
\vspace{1mm}
\begin{tabular}{cccc}
\toprule
\makecell{Latent \\ Prediction} & \cellcolor{gray!30}DS$\uparrow$ & RC$\uparrow$ & IS$\uparrow$ \\ \midrule
$\times$          & \cellcolor{gray!30}67.9$\pm$2.1         & 98.6$\pm$0.8         & 0.68$\pm$0.02         \\
$\checkmark$      & \cellcolor{gray!30}70.1$\pm$2.6 & 97.8$\pm0.9$ & 0.72$\pm$0.03         \\ \bottomrule
\end{tabular}
\label{tab:abl_carla}
\end{wraptable}


==> tables/abl_fix_front.tex <==
\begin{table}[H]
\centering
\caption{\textbf{The importance of  front view.} }
\label{tab:abl_fix_front}
% \resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{l|cccc|cccc}
\toprule
\multirow{2}{*}{Selected Views} & \multicolumn{4}{c|}{L2 (m) $\downarrow$} & \multicolumn{4}{c}{Collision (\%) $\downarrow$} \\
& 1s & 2s & 3s & \cellcolor{gray!30}Avg. & 1s & 2s & 3s & \cellcolor{gray!30}Avg.  \\
\midrule
Two random views  & 0.39 & 0.79 & 1.32 & \cellcolor{gray!30}0.83 & 0.15 & 0.28 & 0.91 & \cellcolor{gray!30}0.45 \\
% \midrule
Front + a random view & 0.36 & 0.74 & 1.24 & \cellcolor{gray!30}0.78 & 0.16 & 0.28 & 0.82 & \cellcolor{gray!30}0.42  \\
\bottomrule
\end{tabular}%
% }
\end{table}
